OED: Towards One-stage End-to-End Dynamic Scene Graph Generation

Dynamic Scene Graph Generation (DSGG) focuses on identifying visual relationships within the spatial-temporal domain of videos. Conventional approaches often employ multi-stage pipelines, which typically consist of object detection, temporal association, and multi-relation classification. However, these methods exhibit inherent limitations due to the separation of multiple stages, and independent optimization of these sub-problems may yield sub-optimal solutions. To remedy these limitations, we propose a one-stage end-to-end framework, termed OED, which streamlines the DSGG pipeline. This framework reformulates the task as a set prediction problem and leverages pair-wise features to represent each subject-object pair within the scene graph. Moreover, another challenge of DSGG is capturing temporal dependencies, we introduce a Progressively Refined Module (PRM) for aggregating temporal context without the constraints of additional trackers or handcrafted trajectories, enabling end-to-end optimization of the network. Extensive experiments conducted on the Action Genome benchmark demonstrate the effectiveness of our design. The code and models are available at \url{https://github.com/guanw-pku/OED}.

==> figures/reb_fig1_each_class.tex <==
\begin{figure}[t]
    \captionsetup{font=footnotesize}
    \setlength{\abovecaptionskip}{0cm} % 调整间距
    \setlength{\belowcaptionskip}{-0.3cm}
    \caption{Performance under With Constraint with mR@50.}
    \includegraphics[width=\linewidth]{figures/imgs/reb_fig1_each_class.png}
\label{fig:reb_each_class}
\vspace{-32pt}
\end{figure}

==> figures/supp_fig1_prm.tex <==
\begin{figure*}[!t]
    \includegraphics[width=\linewidth]{figures/imgs/supp_fig1_prm_revise.pdf}
    \caption{Zoom in Progressively Refined Module.}
\label{fig:supp_prm}
\end{figure*}

==> figures/supp_fig2_visual_attn.tex <==
\begin{figure*}[t]
    \includegraphics[width=\linewidth]{figures/imgs/supp_fig2_visual_attn.pdf}
    \caption{Visualization of attention maps of pair-wise instance feature and pair-wise relation feature.}
\label{fig:supp_visual_attn}
\end{figure*}

==> figures/supp_fig3_scene_graph.tex <==
\begin{figure*}[htpb]
    \includegraphics[width=\linewidth]{figures/imgs/supp_fig3_scene_graph.pdf}
    \caption{Part of predictions of our Spatial Context Aggregation and Spatial-Temporal Context Aggregation under \textit{with constraint} setting, which match with ground truth.}
\label{fig:supp_scene_graph}
\end{figure*}

==> sections/4_table/1_sota_back.tex <==
\begin{table*}[tb!]
\centering
\caption{Comparison with state-of-the-art scene graph generation methods on Action Genome.   
% Note that * denotes that adopted backbone is ResNet-50, while others depend on ResNet-101.
}
\setlength{\tabcolsep}{2pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{c ccccccccc ccccccccc}
\toprule
  & \multicolumn{9}{c}{With Constraint} & \multicolumn{9}{c}{No Constraints}\\
  \cmidrule(lr){2-10} \cmidrule(lr){11-19}
  Method  &
   \multicolumn{3}{c}{SGDET} & \multicolumn{3}{c}{SGCLS} &  \multicolumn{3}{c}{PredCLS} & \multicolumn{3}{c}{SGDET} & \multicolumn{3}{c}{SGCLS} & \multicolumn{3}{c}{PredCLS}\\ 
   \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}
   & R@10 & R@20 & R@50 & R@10 & R@20 & R@50 & R@10 & R@20 & R@50  & R@10 & R@20 & R@50 & R@10 & R@20 & R@50  & R@10 & R@20 & R@50 \\
% \midrule
\midrule
VRD~~\cite{lu2016visual}   &19.2 &24.5 &26.0 & 32.4 &33.3 &33.3 &51.7 &54.7 &54.7 &19.1 &28.8 &40.5 &39.2 &49.8 &52.6 &59.6 &78.5 &99.2 \\
MSDN~\cite{li2017scene} &24.1 &32.4 &34.5 &43.9 &45.1 &45.1 &65.5 &68.5 &68.5 &23.1 &34.7 &46.5 &51.2& 61.8 &65.0 &74.9 &92.7 &99.0 \\
M-FREQ~\cite{zellers2018neural} &23.7 &31.4 &33.3 &40.8 &41.9 &41.9 &62.4 &65.1 &65.1 &22.8 &34.3 &46.4 &50.4 &60.6 &64.2 &73.4 &92.4 &99.6 \\
VCTree~\cite{tang2019learning} &24.4 &32.6 &34.7 &44.1 &45.3 &45.3 &66.0 &69.3 &69.3 &23.9 &35.3 &46.8 &52.4 &62.0 &65.1 &75.5 &92.9 &99.3 \\
RelDN~\cite{zhang2019graphical} &24.5 &32.8 &34.9 &44.3 &45.4 &45.4 &66.3 &69.5 &69.5 &24.1 &35.4 &46.8 &52.9 &62.4 &65.1 &75.7 &93.0 & 99.0 \\
GPS-Net~\cite{lin2020gps} &24.7 &33.1 &35.1 &45.3 &46.5 &46.5 &66.8 &69.9 &69.9 &24.4 &35.7 &47.3 &53.6 &63.3 &66.0 &76.0 &93.6 &99.5 \\
TRACE~\cite{teng2021target} &13.9 &14.5 &14.5 &14.8 &14.8 &14.8 &27.5 &27.5 &27.5 &26.5 &35.6 &45.3 &37.1 &46.7 &50.5 &72.6 &91.6 &96.4 \\
STTran~\cite{cong2021spatial} &25.2 &34.1 &37.0 &46.4 &47.5 &47.5 &68.6 &71.8 &71.8 &24.6 &36.2 &48.8 &54.0 &63.7 &66.4 &77.9 &94.2 &99.1 \\
APT~\cite{li2022dynamic} &26.3 & \underline{36.1} & \underline{38.3} &47.2 &48.9 &48.9 &69.4 &73.8 & 73.8 &25.7 &37.9 &\underline{50.1} &55.1 &65.1 &68.7 &78.5 &95.1 &99.2 \\
STTran-TPI~\cite{wang2022dynamic} &26.2 &34.6 &37.4 &47.2 &48.3 &48.3 &69.7 &72.6 &72.6 &- &- &- &- &- &- &- &- &- \\
TR$^2$~\cite{wang2023cross} &26.8 &35.5 &38.3 &47.7 &48.7 &48.7 &70.9 &73.8 &73.8 &27.8 &39.2 &50.0 &57.2 &64.4 &66.2 &83.1 &96.6 &99.9 \\
TEMPURA~\cite{nag2023unbiased} &28.1 &33.4 &34.9 &47.2 &48.3 &48.3 &68.8 &71.5 &71.5 &29.8 &38.1 &46.4 &56.3 &64.7 &67.9 &80.4 &94.2 &99.4 \\
DSG-DETR~\cite{feng2023exploiting} &\underline{30.3} &34.8 &36.1 &50.8 &52.0 &52.0 &- &- &- &\underline{32.1} &\underline{40.9} &48.3 &59.2 &69.1 &72.4 &- &- &- \\
% TPT*~\cite{zhang2023end} &- &- &- &- &- &- &- &- &- &29.6 &37.3 &49.2 &- &- &- &85.5 &97.3 &99.9 \\
TPT~\cite{zhang2023end} &- &- &- &- &- &- &- &- &- &32.0 &39.6 &\bf 51.5 &- &- &- &\bf 85.6 &\bf 97.4 &\bf 99.9 \\
Ours &\bf 33.5 &\bf 40.7 &\bf 47.3 & & & &\bf 72.9 &\bf 76.0 &\bf 76.1 &\bf 35.3 &\bf 43.5 &\underline{50.1} &&&& \underline{83.3} &95.4 &99.2 \\

\bottomrule
\end{tabular}
}
\end{table*}


==> sections/4_table/2_ablation_design.tex <==
\begin{table*}[htbp]
    \centering
    \setlength{\tabcolsep}{2pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|cccccc|ccc|ccc}
    \toprule
    \multirow{2}{*}{\makecell[c]{\#}} &
    \multirow{2}{*}{\makecell[c]{Spatial \\ Baseline}} &
    \multirow{2}{*}{\makecell[c]{Cascaded \\ Decoders}} &
    \multirow{2}{*}{\makecell[c]{Matched \\ Loss}} & 
    \multirow{2}{*}{\makecell[c]{Triplet \\ Interaction}} &
    \multirow{2}{*}{\makecell[c]{Progressively \\ Refined Interaction}} & 
    \multirow{2}{*}{\makecell[c]{Triplet \\ NMS Filter}} & 
    \multicolumn{3}{c|}{With Constraint} & \multicolumn{3}{c}{No Constraints} \\
    &&&&&&&R@10 &R@20 &R@50 &R@10 &R@20 &R@50 \\
    \midrule
    1 & \checkmark&&&&& &26.3 &29.2	&32.1 &28.4 &32.9	&37.2 \\
    2 & \checkmark &\checkmark  &&&& &27.2 &30.3 &33.7 &29.2 &34.0 &38.4 \\
    3 & \checkmark &\checkmark &\checkmark &&& &31.5 &37.7 &43.7 &33.4 &41.6 &49.0 \\
    4 & \checkmark &\checkmark &\checkmark &\checkmark && &31.7 &37.9 &44.0 &33.6 &41.8 &49.2 \\
    5 & \checkmark &\checkmark &\checkmark &\checkmark & \checkmark & &32.8 &39.0 &45.0 &34.7 &42.9 &50.3 \\
    6 & \checkmark &\checkmark &\checkmark &\checkmark &\checkmark &\checkmark &33.5 &40.9 &48.9 &35.3 &44.0 & 51.8 \\
    \bottomrule
    \end{tabular}}
    \caption{Ablation studies on different designs for scene graph detection task.}
    \label{tab:ablation_design}
\end{table*}

==> sections/4_table/5_long_tail.tex <==
\begin{table}[h!]
\captionsetup{font=footnotesize}
% \fontsize{40.5}{13.8}\selectfont
\renewcommand{\arraystretch}{1}
% \setlength{\abovecaptionskip}{0cm} % 调整间距
% \setlength{\belowcaptionskip}{-0.4cm}
\Huge
\centering
\caption{Performance comparison under Mean Recall and Head-body-tail classes with mR@50.}
% \setlength{\tabcolsep}{1pt}
% \setlength{\arraystretch}{0.5}{
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{c|c|c|c|c}
\toprule
  \multirow{2}{*}{Method} & \multicolumn{2}{c|}{With Constraint} & \multicolumn{2}{c}{No Constraints} \\ 
    &mR@10/20/50  &Head/Body/Tail  &mR@10/20/50  &Head/Body/Tail\\
% \midrule
\midrule
STTran[4]	&16.5/20.8/22.2 &\underline{39.00}/25.53/12.78 &20.9/29.6/39.1 &\underline{45.39}/52.32/26.67 \\
DSG-DETR[8] &18.0/21.3/22.0 &37.91/\underline{25.84}/12.62 &23.6/30.1/36.5 &44.76/\underline{52.65}/21.09 \\
TEMPURA[19] &\underline{18.4}/\underline{22.5}/\underline{23.6} &36.53/23.79/\underline{18.15} &\underline{24.5}/\underline{33.8}/\underline{43.6} &42.50/50.66/\underline{38.86} \\
Ours &\textbf{20.9}/\textbf{26.9}/ \textbf{32.9} &\textbf{51.44}/\textbf{36.38}/\textbf{22.72} &\textbf{26.3}/\textbf{39.5}/\textbf{49.5} &\textbf{48.75}/\textbf{56.12}/\textbf{44.89} \\

\bottomrule
\end{tabular}
}
\label{tab:long_tail}
% \vspace{-13pt}
\end{table}


==> sections/4_table/x_rebuttal.tex <==
\begin{table*}[htbp]
\tiny
\centering
\caption{}
\setlength{\tabcolsep}{2pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{c| cccccc| cccccc| cc| c}
\toprule
  \multirow{2}{*}{Method} & \multicolumn{6}{c|}{With Constraint} & \multicolumn{6}{c|}{No Constraints} &\multicolumn{2}{c|}{Efficiency} & Computation \\ 
                %\cmidrule(lr){2-16}
  
    &R@10 &mR@10 &R@20 &mR@20 &R@50 &mR@50 &R@10 &mR@10 &R@20 &mR@20 &R@50 &mR@50 &Time &FPS &FLOPs\\
% \midrule
\midrule

STTran[4]	&25.2	&16.5	&34.0	&20.8	&36.9	&22.2	&24.5	&20.9	&36.1	&29.6	&48.8	&39.1	&30.71 ms	&32.48 	&126.27 G \\
TEMPURA[19] &28.0	&18.4	&33.3	&22.5	&34.8	&23.6	&29.8	&24.5	&38.0	&33.8	&46.3	&43.6	&30.32 ms	&32.97 	&126.53 G\\
DSG-DETR[8] &30.4 &18.0 &34.9 &21.3 &36.0 &22.0 &32.3 &23.6 &40.9 &30.1 &48.2 &36.5 &36.74 ms &27.22  &\\
TPT[38] &- &- &- &- &- &- &32.0 &- &39.6 &- &51.5 &- &*71.32 ms	&*14.02  &-\\
Ours &33.5 &20.9 &40.9 &26.9 &48.9 &32.9 &35.3 &26.3 &44.0 &39.5 &51.8 &49.5 &43.31 ms &23.09 &156.85 G \\

\bottomrule
\end{tabular}
}
\label{tab:rebuttal}
\end{table*}


==> sections/4_table/x_rebuttal_efficiency.tex <==
% \begin{table}[htbp!]
% \setlength{\abovecaptionskip}{0cm} % 调整间距
% \setlength{\belowcaptionskip}{-0.3cm}
% \tiny
% \centering
% \captionsetup{font=footnotesize}
% \caption{Complexity comparisons.}
% \setlength{\tabcolsep}{2pt}
% \resizebox{0.3\textwidth}{!}{
% \begin{tabular}{c|c|c|c|c|c}
% \toprule
%   Method & Time Complexity \downarrow & Time \downarrow & FPS \uparrow & Params \downarrow & SGDET-R@50 \uparrow \\
% \midrule
% STTran[4] &$O(MN^2)$ &29.4 ms &33.9 &103.3M & 37.0\\
% DSG-DETR[8] &$O(MN^2)$ &36.3 ms &27.5 &186.1M & 36.1\\ % &36.74 ms &27.22 & \\
% TEMPURA[19] &$O(MN^2)$ &30.5 ms &32.7 &201.1M & 34.9\\ % &30.32 ms &32.97 & \\
% Ours &$O(MN)$ &\textbf{16.9 ms} &\textbf{59.1} &\textbf{63.7M} & \textbf{48.9}\\ % &43.31 ms &23.09 & \\
% \bottomrule
% \end{tabular}
% }
% \vspace{-12pt}
% \label{tab:rebuttal_efficiency}
% \end{table}


\begin{table}[htbp!]
\setlength{\abovecaptionskip}{0cm} % 调整间距
\setlength{\belowcaptionskip}{-0.4cm}
\Huge
\centering
\captionsetup{font=footnotesize}
\caption{Complexity comparisons on Action Genome in SGDET task.}
% \yang{which dataset?}\yang{change metric to R@10}.}
\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{10pt}
\resizebox{0.43\textwidth}{!}{
\begin{tabular}{c|c|c|c|c}
\toprule
  Method & Complexity & FPS & Params/M & SGDET-R@10 \\
\midrule
STTran[4] &$O(MN^2)$  &33.9~\color{red}({-25.2}) &103.3~\color{red}{(+39.6)} & 24.6~\color{red}{(-10.9)}\\
TEMPURA[19] &$O(MN^2)$  &32.7~\color{red}({-26.4}) &201.1~\color{red}{(+137.4)} & 29.8~\color{red}{(-5.5)}\\ % &30.32 ms &32.97 & \\
DSG-DETR[8] &$O(MN^2)$ &27.5~\color{red}({-31.6}) &186.1~\color{red}{(+122.4)} & 32.1~\color{red}{(-3.2)}\\ % &36.74 ms &27.22 & \\
Ours &$O(KM)$  &\textbf{59.1} &\textbf{63.7} & \textbf{35.3}\\ % &43.31 ms &23.09 & \\
\bottomrule
\end{tabular}
}
\vspace{-13pt}
\label{tab:rebuttal_efficiency}
\end{table}


==> sections/4_table/x_rebuttal_head_body_tail.tex <==
\begin{table}[htbp!]
% \tiny
\captionsetup{font=footnotesize}
\setlength{\abovecaptionskip}{0cm} % 调整间距
\setlength{\belowcaptionskip}{-0.3cm}
\centering
\caption{Performance on head-body-tail classes with mR@50.}
\setlength{\tabcolsep}{2pt}
\resizebox{0.28\textwidth}{!}{
\begin{tabular}{c| ccc| ccc}
\toprule
  \multirow{2}{*}{Method} & \multicolumn{3}{c|}{With Constraint} & \multicolumn{3}{c}{No Constraints} \\
    &Head &Body &Tail &Head &Body &Tail \\
% \midrule
\midrule

STTran[4] &\underline{39.00} &25.53 &12.78 &\underline{45.39} &52.32 &26.67 \\
DSG-DETR[8] &37.91 &\underline{25.84} &12.62 &44.76 &\underline{52.65} &21.09 \\
TEMPURA[19] &36.53 &23.79 &\underline{18.15} &42.50 &50.66 &\underline{38.86}\\
Ours &\textbf{51.44} &\textbf{36.38} &\textbf{22.72} &\textbf{48.75} &\textbf{56.12} &\textbf{44.89} \\
\bottomrule
\end{tabular}
}
\label{tab:rebuttal_head_body_tail}
\vspace{-13pt}
\end{table}


==> sections/4_table/x_rebuttal_mrecall.tex <==
% \begin{table}[htbp!]
% \tiny
% \centering
% \caption{}
% \setlength{\tabcolsep}{1pt}
% \resizebox{0.5\textwidth}{!}{
% \begin{tabular}{c| cccccc| cccccc}
% \toprule
%   \multirow{2}{*}{Method} & \multicolumn{6}{c|}{With Constraint} & \multicolumn{6}{c}{No Constraints} \\ 
%     &R@10 &mR@10 &R@20 &mR@20 &R@50 &mR@50 &R@10 &mR@10 &R@20 &mR@20 &R@50 &mR@50 \\
% % \midrule
% \midrule
% STTran	&25.2	&16.5	&34.0	&20.8	&36.9	&22.2	&24.5	&20.9	&36.1	&29.6	&48.8	&39.1 \\
% DSG-DETR &30.4 &18.0 &34.9 &21.3 &36.0 &22.0 &32.3 &23.6 &40.9 &30.1 &48.2 &36.5 \\
% TEMPURA &28.0	&18.4	&33.3	&22.5	&34.8	&23.6	&29.8	&24.5	&38.0	&33.8	&46.3	&43.6 \\
% Ours &33.5 &20.9 &40.9 &26.9 &48.9 &32.9 &35.3 &26.3 &44.0 &39.5 &51.8 &49.5 \\

% \bottomrule
% \end{tabular}
% }
% \label{tab:rebuttal}
% \end{table}


% \begin{table}[h!]
% \captionsetup{font=footnotesize}
% \fontsize{40.5}{13.8}\selectfont
% \renewcommand{\arraystretch}{1}
% \setlength{\abovecaptionskip}{0cm} % 调整间距
% \setlength{\belowcaptionskip}{-0.3cm}
% \Huge
% \centering
% \caption{Performance with both Recall and Mean Recall metrics.}
% % \setlength{\tabcolsep}{1pt}
% % \setlength{\arraystretch}{0.5}{
% \resizebox{0.48\textwidth}{!}{
% \begin{tabular}{c| cccccc| cccccc}
% \toprule
%   \multirow{2}{*}{Method} & \multicolumn{6}{c|}{With Constraint} & \multicolumn{6}{c}{No Constraints} \\ 
%     &R@10 &R@20 &R@50 &mR@10 &mR@20 &mR@50 &R@10 &R@20 &R@50 &mR@10 &mR@20 &mR@50 \\
% % \midrule
% \midrule
% STTran[4]	&25.2	&34.0  &\underline{36.9} &16.5  &20.8 &22.2	&24.5	&36.1  &\underline{48.8}  &20.9	 &29.6	&39.1 \\
% DSG-DETR[8] &\underline{30.4} &\underline{34.9} &36.0 &18.0  &21.3  &22.0 &\underline{32.3} &\underline{40.9} &48.2 &23.6 &30.1 &36.5 \\
% TEMPURA[19] &28.0 &33.3 &34.8 &\underline{18.4} &\underline{22.5} &\underline{23.6}	&29.8 &38.0 &46.3 &\underline{24.5} &\underline{33.8} &\underline{43.6} \\
% Ours &\textbf{33.5} &\textbf{40.9} &\textbf{48.9} &\textbf{20.9} &\textbf{26.9} &\textbf{32.9} &\textbf{35.3} &\textbf{44.0} &\textbf{51.8} &\textbf{26.3} &\textbf{39.5} &\textbf{49.5} \\

% \bottomrule
% \end{tabular}
% }
% \label{tab:rebuttal_mrecall}
% \vspace{-14pt}
% \end{table}



\begin{table}[h!]
\captionsetup{font=footnotesize}
% \fontsize{40.5}{13.8}\selectfont
\renewcommand{\arraystretch}{1}
\setlength{\abovecaptionskip}{0cm} % 调整间距
\setlength{\belowcaptionskip}{-0.4cm}
\Huge
\centering
\caption{Performance with both Recall and Mean Recall metrics.}
% \setlength{\tabcolsep}{1pt}
% \setlength{\arraystretch}{0.5}{
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{c|c|c|c|c}
\toprule
  \multirow{2}{*}{Method} & \multicolumn{2}{c|}{With Constraint} & \multicolumn{2}{c}{No Constraints} \\ 
    &R@10/20/50 &mR@10/20/50 &R@10/20/50 &mR@10/20/50 \\
% \midrule
\midrule
STTran[4]	&25.2/34.0/\underline{36.9} &16.5/20.8/22.2	&24.5/36.1/\underline{48.8}  &20.9/29.6/39.1 \\
DSG-DETR[8] &\underline{30.4}/\underline{34.9}/36.0 &18.0/21.3/22.0 &\underline{32.3}/\underline{40.9}/48.2 &23.6/30.1/36.5 \\
TEMPURA[19] &28.0/33.3/34.8 &\underline{18.4}/\underline{22.5}/\underline{23.6}	&29.8/38.0/46.3 &\underline{24.5}/\underline{33.8}/\underline{43.6} \\
Ours &\textbf{33.5}/\textbf{40.9}/\textbf{48.9} &\textbf{20.9}/\textbf{26.9}/ \textbf{32.9} &\textbf{35.3}/\textbf{44.0}/\textbf{51.8} &\textbf{26.3}/\textbf{39.5}/\textbf{49.5} \\

\bottomrule
\end{tabular}
}
\label{tab:rebuttal_mrecall}
\vspace{-13pt}
\end{table}


==> sections/4_table/x_rebuttal_sgg.tex <==
\begin{table}[htbp!]
\captionsetup{font=footnotesize}
\setlength{\abovecaptionskip}{0cm} % 调整间距
\setlength{\belowcaptionskip}{-0.3cm}
% \tiny
\centering
\caption{Performance of image-base one-stage methods.}
\setlength{\tabcolsep}{2pt}
\resizebox{0.28\textwidth}{!}{
\begin{tabular}{c|c| ccc| ccc}
\toprule
  \multirow{2}{*}{Line} & \multirow{2}{*}{Method} & \multicolumn{3}{c|}{With Constraint} & \multicolumn{3}{c}{No Constraints} \\
    & &R@10 &R@20 &R@50 &R@10 &R@20 &R@50 \\
% \midrule
\midrule
1 &RelTR &19.7 &23.4 &25.9 &20.9 &24.6 &28.2\\
2 &RelTR+M &20.1 &24.9 &28.0 &21.8 &28.0 &32.7 \\ 
3 &RelTR+M+P &23.5 &28.6 &31.9 &25.0 &31.8 &36.8 \\
4 &Ours &\textbf{33.5} &\textbf{40.9} &\textbf{48.9} &\textbf{35.3} &\textbf{44.0} &\textbf{51.8} \\

% Ours &\textbf{51.44} &\textbf{36.38} &\textbf{22.72} &\textbf{48.75} &\textbf{56.12} &\textbf{44.89} \\
\bottomrule
\end{tabular}
}
\label{tab:rebuttal_sgg}
\vspace{-13pt}
\end{table}



==> sections/4_table/x_rebuttal_sgg_long_tail.tex <==


% 在当前栏内放置两个并排的表格
% \begin{table}[htbp] % 通常会用浮动环境来管理表格的位置
% \captionsetup{font=footnotesize}
% \Huge
% \renewcommand{\arraystretch}{1.2}
% \setlength{\abovecaptionskip}{0cm} % 调整间距
% \setlength{\belowcaptionskip}{-0.25cm}
% \begin{minipage}[t]{0.52\linewidth}
% \centering
% \captionsetup{type=table}% 设置caption类型为表格
% \caption{Image-based SGG methods.}\label{tab:rebuttal_sgg}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c|c| ccc| ccc}
% \toprule
%   \multirow{2}{*}{\#} & \multirow{2}{*}{Method} & \multicolumn{3}{c|}{With Constraint} & \multicolumn{3}{c}{No Constraints} \\
%     &&R@10 &R@20 &R@50 &R@10 &R@20 &R@50 \\
% % \midrule
% \midrule
% 1&RelTR[5] &19.7 &23.4 &25.9 &20.9 &24.6 &28.2\\
% 2&RelTR+M &20.1 &24.9 &28.0 &21.8 &28.0 &32.7 \\ 
% 3&RelTR+M+P &23.5 &28.6 &31.9 &25.0 &31.8 &36.8 \\
% 4&Ours &\textbf{33.5} &\textbf{40.9} &\textbf{48.9} &\textbf{35.3} &\textbf{44.0} &\textbf{51.8} \\

% % Ours &\textbf{51.44} &\textbf{36.38} &\textbf{22.72} &\textbf{48.75} &\textbf{56.12} &\textbf{44.89} \\
% \bottomrule
% \end{tabular}
% }
% \end{minipage}%
% \hfill
% \begin{minipage}[t]{0.48\linewidth}
% \centering
% \captionsetup{type=table}
% \caption{Head-body-tail classes.}\label{tab:rebuttal_head_body_tail}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c| ccc| ccc}
% \toprule
%   \multirow{2}{*}{Method} & \multicolumn{3}{c|}{With Constraint} & \multicolumn{3}{c}{No Constraints} \\
%     &Head &Body &Tail &Head &Body &Tail \\
% % \midrule
% \midrule
% STTran[4] &\underline{39.00} &25.53 &12.78 &\underline{45.39} &52.32 &26.67 \\
% DSG-DETR[8] &37.91 &\underline{25.84} &12.62 &44.76 &\underline{52.65} &21.09 \\
% TEMPURA[19] &36.53 &23.79 &\underline{18.15} &42.50 &50.66 &\underline{38.86}\\
% Ours &\textbf{51.44} &\textbf{36.38} &\textbf{22.72} &\textbf{48.75} &\textbf{56.12} &\textbf{44.89} \\
% \bottomrule
% \end{tabular}
% }
% \end{minipage}
% \vspace{-14.5pt}
% \end{table}



\begin{table}[htbp] % 通常会用浮动环境来管理表格的位置
\captionsetup{font=footnotesize}
\Huge
\renewcommand{\arraystretch}{1.2}
\setlength{\abovecaptionskip}{0cm} % 调整间距
\setlength{\belowcaptionskip}{-0.4cm}
\begin{minipage}[t]{0.475\linewidth}
\centering
\captionsetup{type=table}% 设置caption类型为表格
\caption{Image-based methods.}\label{tab:rebuttal_sgg}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|c|c}
\toprule
  \multirow{2}{*}{\#} & \multirow{2}{*}{Method} & \multicolumn{1}{c|}{With Constraint} & \multicolumn{1}{c}{No Constraints} \\
    &&R@10/20/50  &R@10/20/50 \\
% \midrule
\midrule
1&RelTR[5] &19.7/23.4/25.9 &20.9/24.6/28.2\\
2&RelTR+M &20.1/24.9/28.0 &21.8/28.0/32.7 \\ 
3&RelTR+M+P &23.5/28.6/31.9 &25.0/31.8/36.8 \\
4&Ours &\textbf{33.5}/\textbf{40.9}/\textbf{48.9} &\textbf{35.3}/\textbf{44.0}/\textbf{51.8} \\

% Ours &\textbf{51.44} &\textbf{36.38} &\textbf{22.72} &\textbf{48.75} &\textbf{56.12} &\textbf{44.89} \\
\bottomrule
\end{tabular}
}
\end{minipage}%
\hfill
\begin{minipage}[t]{0.525\linewidth}
\centering
\captionsetup{type=table}
\caption{Head-body-tail classes.}\label{tab:rebuttal_head_body_tail}
\resizebox{\textwidth}{!}{
\begin{tabular}{c| c| c}
\toprule
  \multirow{2}{*}{Method} & \multicolumn{1}{c|}{With Constraint} & \multicolumn{1}{c}{No Constraints} \\
    &Head/Body/Tail &Head/Body/Tail \\
% \midrule
\midrule
STTran[4] &\underline{39.00}/25.53/12.78 &\underline{45.39}/52.32/26.67 \\
DSG-DETR[8] &37.91/\underline{25.84}/12.62 &44.76/\underline{52.65}/21.09 \\
TEMPURA[19] &36.53/23.79/\underline{18.15} &42.50/50.66/\underline{38.86}\\
Ours &\textbf{51.44}/\textbf{36.38}/\textbf{22.72} &\textbf{48.75}/\textbf{56.12}/\textbf{44.89} \\
\bottomrule
\end{tabular}
}
\end{minipage}
\vspace{-14.5pt}
\end{table}







% % 在当前栏内放置两个并排的表格
% \begin{table}[htbp] % 通常会用浮动环境来管理表格的位置
% \captionsetup{font=footnotesize}
% \Huge
% \renewcommand{\arraystretch}{1.2}
% \setlength{\abovecaptionskip}{0cm} % 调整间距
% \setlength{\belowcaptionskip}{-0.25cm}
% \begin{minipage}[t]{0.52\linewidth}
% \centering
% \captionsetup{type=table}% 设置caption类型为表格
% \caption{Image-based SGG methods.}\label{tab:rebuttal_sgg}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c|c| c| c}
% \toprule
%   \multirow{2}{*}{\#} & \multirow{2}{*}{Method} & With Constraint & No Constraints \\
%   &&&(R@10/20/50)&(R@10/20/50) \\
% % \midrule
% \midrule
% 1&RelTR[5] &19.7/23.4/25.9 &20.9/24.6/28.2\\
% % 2&RelTR+M &20.1 &24.9 &28.0 &21.8 &28.0 &32.7 \\ 
% % 3&RelTR+M+P &23.5 &28.6 &31.9 &25.0 &31.8 &36.8 \\
% % 4&Ours &\textbf{33.5} &\textbf{40.9} &\textbf{48.9} &\textbf{35.3} &\textbf{44.0} &\textbf{51.8} \\

% % Ours &\textbf{51.44} &\textbf{36.38} &\textbf{22.72} &\textbf{48.75} &\textbf{56.12} &\textbf{44.89} \\
% \bottomrule
% \end{tabular}
% }
% \end{minipage}%
% \hfill
% \begin{minipage}[t]{0.48\linewidth}
% \centering
% \captionsetup{type=table}
% \caption{Head-body-tail classes.}\label{tab:rebuttal_head_body_tail}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c| ccc| ccc}
% \toprule
%   \multirow{2}{*}{Method} & \multicolumn{3}{c|}{With Constraint} & \multicolumn{3}{c}{No Constraints} \\
%     &Head &Body &Tail &Head &Body &Tail \\
% % \midrule
% \midrule
% STTran[4] &\underline{39.00} &25.53 &12.78 &\underline{45.39} &52.32 &26.67 \\
% DSG-DETR[8] &37.91 &\underline{25.84} &12.62 &44.76 &\underline{52.65} &21.09 \\
% TEMPURA[19] &36.53 &23.79 &\underline{18.15} &42.50 &50.66 &\underline{38.86}\\
% Ours &\textbf{51.44} &\textbf{36.38} &\textbf{22.72} &\textbf{48.75} &\textbf{56.12} &\textbf{44.89} \\
% \bottomrule
% \end{tabular}
% }
% \end{minipage}
% \vspace{-14.5pt}
% \end{table}


==> sections/4_table/x_supp_long-tail.tex <==
\begin{table*}[h!]
\captionsetup{font=footnotesize}
% \fontsize{40.5}{13.8}\selectfont
\renewcommand{\arraystretch}{1}
% \setlength{\abovecaptionskip}{0cm} % 调整间距
% \setlength{\belowcaptionskip}{-0.4cm}
\Huge
\centering
\caption{Performance comparison under both Recall and Mean Recall Metrics and Head-body-tail classes with mR@50.}
% \setlength{\tabcolsep}{1pt}
% \setlength{\arraystretch}{0.5}{
\resizebox{\textwidth}{!}{
\begin{tabular}{c ccc|ccc|ccc | ccc|ccc|ccc}
\toprule
  & \multicolumn{9}{c|}{With Constraint} & \multicolumn{9}{c}{No Constraints} \\ 
  \cmidrule(lr){2-10} \cmidrule(lr){11-19}
  Method
    &R@10 &R@20 &R50 &mR@10 &mR@20 &mR50  &Head &Body &Tail &R@10 &R@20 &R50 &mR@10 &m20 &mR50  &Head &Body &Tail\\
% \midrule
\midrule

STTran~\cite{cong2021spatial}	&25.2 &34.0 &\underline{36.9} &16.5 &20.8 &22.2 &\underline{39.00} &25.53 &12.78  &24.5 &36.1 &\underline{48.8} &20.9 &29.6 &39.1 &\underline{45.39} &52.32 &26.67 \\
DSG-DETR~\cite{feng2023exploiting} &\underline{30.4} &\underline{34.9} &36.0 &18.0 &21.3 &22.0 &37.91 &\underline{25.84} &12.62 &\underline{32.3} &\underline{40.9} &48.2 &23.6 &30.1 &36.5 &44.76 &\underline{52.65} &21.09 \\
TEMPURA~\cite{nag2023unbiased} &28.0 &33.3 &34.8 &\underline{18.4} &\underline{22.5} &\underline{23.6} &36.53 &23.79 &\underline{18.15} &29.8 &38.0 &46.3 &\underline{24.5} &\underline{33.8} &\underline{43.6} &42.50 &50.66 &\underline{38.86} \\
Ours &\textbf{33.5} &\textbf{40.9} &\textbf{48.9} &\textbf{20.9} &\textbf{26.9} & \textbf{32.9} &\textbf{51.44} &\textbf{36.38} &\textbf{22.72} &\textbf{35.3} &\textbf{44.0} &\textbf{51.8} &\textbf{26.3} &\textbf{39.5} &\textbf{49.5} &\textbf{48.75} &\textbf{56.12} &\textbf{44.89} \\

\bottomrule
\end{tabular}
}
\label{tab:supp_long_tail}
% \vspace{-13pt}
\end{table*}

